Orientation-Aware Graph Neural Networks for Protein Structure Representation Learning

By folding into particular 3D structures, proteins play a key role in living beings. To learn meaningful representation from a protein structure for downstream tasks, not only the global backbone topology but the local fine-grained orientational relations between amino acids should also be considered. In this work, we propose the Orientation-Aware Graph Neural Networks (OAGNNs) to better sense the geometric characteristics in protein structure (e.g. inner-residue torsion angles, inter-residue orientations). Extending a single weight from a scalar to a 3D vector, we construct a rich set of geometric-meaningful operations to process both the classical and SO(3) representations of a given structure. To plug our designed perceptron unit into existing Graph Neural Networks, we further introduce an equivariant message passing paradigm, showing superior versatility in maintaining SO(3)-equivariance at the global scale. Experiments have shown that our OAGNNs have a remarkable ability to sense geometric orientational features compared to classical networks. OAGNNs have also achieved state-of-the-art performance on various computational biology applications related to protein 3D structures. The code is available at https://github.com/Ced3-han/OAGNN/tree/main.

==> sections/20-related.tex <==
\section{Related Work}

\textbf{Representation learning on protein 3D structure.}
Early approaches rely on hand-crafted features extracted and statistical methods to predict function annotations \cite{schaap2001rosetta,zhang2010novel}. Deep learning has been found to achieve success then. 3D CNNs are first proposed to process protein 3D structures by scanning atom-level features relying on multiple 3D voxels. One of the representative works \cite{derevyanko2018deep} adopts a 3D CNN-based model for assessing the quality of the predicted structures. 3D CNNs also shed light on other tasks such as interface prediction \cite{townshend2019end,amidi2018enzynet}. People also extend them to spherical convolutions \cite{gainza2020deciphering,sverrisson2021fast,hermosilla2021intrinsic}, to the Fourier space \cite{zhemchuzhnikov20216dcnn} and the 3D Voronoi Tessellation space \cite{igashov2021vorocnn}. Graph Convolutional Networks \cite{kipf2016semi} has also been adopted to capture geometric and biochemical interactions between residues \cite{ying2018hierarchical,gao2019graph,fout2017protein}, and have been shown to achieve great performance on function prediction \cite{li2021structure}, protein design \cite{strokach2020fast} and binding prediction \cite{vecchio2021neural}. Recently, transformer-based methods \cite{vaswani2017attention} have a trend to replace conventional methods in other bioinformatics tasks \cite{ingraham2019generative,baek2021accurate,jumper2021highly,cao2021fold2seq}.

\textbf{Equivariant neural networks.}
Equivariance is an important property, for generalizing to unseen conditions in geometric learning. \cite{cohen2016group,weiler20183d,kohler2020equivariant,satorras2021n,thomas2018tensor,fuchs2020se,anderson2019cormorant,klicpera2020directional,batzner2021se,eismann2021hierarchical}. Methods such as Tensor Field Network \cite{thomas2018tensor} and Cormorant \cite{anderson2019cormorant}, have been developed to generate irreducible representations for achieving rotation equivariance in 3D. In comparison to the Tensor Filed Network with complex tensor products, the Vector Neuron Network (VNN) achieves rotation equivariance in a much simpler way, which generalizes the values of hidden neurons from scalars to 3D vectors \cite{deng2021vector}. GVP-GNN has also been introduced for learning protein representations by featuring geometric factors as vectors \cite{jing2020learning}. Message passing in GNNs for vector representations using equivariant features have also been explored \cite{schutt2021equivariant,luo2022equivariant}. However, to guarantee rotation equivariance, they can only linearly combine 3D vectors, in essence, limiting their geometric representing capacity. Another line of methods condition filters on invariant scalar features for maintaining equivariance \cite{schutt2017schnet,gasteiger2019directional,liu2021spherical}.


%However, they can only linearly combine 3D vectors to satisfy the rotation equivariance, in essence, limiting the model's geometric expressiveness.

==> sections/30-methods_OLD.tex <==
\section{Methods}
\label{dwnn}
We model the entire protein 3D structure as a graph and use the Message Passing Neural Network as the framework to propagate the local information (features for each residue) across nodes. We replace the fully connected perceptrons with the directed weight perceptrons (\Secref{dwp}), and use an equivariant message passing paradigm to update the representations of each node (\Secref{emp}). To enable efficient integration of scalar and vector features, we design a cross-attention layer to selectively integrate geometric features. (\Secref{variants}).


\subsection{Directed Weight Perceptrons}
\label{dwp}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/overview.pdf}
    \caption{
    Task Overview. a) A given residue in a protein has its rigid backbone, and can be represented by both scalar and vector features. b) Two protein representation tasks. MQA evaluates predicted protein structures (graph-level), and CPD generates the protein sequence from the backbone structure (node-level). 
    \CD{Is it better to put a network overview instead of the task overview in the teaser?}
    }
    \label{fig:model_overview}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/detail.pdf}
    \caption{
    Model Details. a) \textbf{Directed Linear Module} applies multiple geometric operations to update scalar and vector features respectively. b) \textbf{Directed Interaction Module} updates the features by using one another as updating parameters.
    \CD{May be better to draw all the three modules so the figure aligns with the text, even the non-linear module is only a small part. Can probably list the three modules in a horizontal sequence (two column figure).}
    \CD{Should swap $\vh$ and $\mH$ in the figure?}
    }
    \label{fig:model_detail}
\end{figure}


We consider a hybrid scalar-vector representation where a neuron (of index $i$) can be either a scalar $s_i \in \mathbb{R}$ or a 3D vector $\vv_i \in \mathbb{R}^3$.
A network feature is then represented as a scalar-vector tuple $(\vs,\mV),\vs \in \mathbb{R}^{C^s},\mV \in \mathbb{R}^{C^v \times 3}$ comprising of $C^s$ scalar neurons and $C^v$ vector neurons.
%
We design our Directed Weight (DW) perceptrons on top of this representation, mapping a scalar-vector tuple $(\vs,\mV)$ to another scalar-vector tuple $(\vs',\mV')$.



We introduce three basic computation modules, serving as building blocks for each DW layer: the \textbf{Directed Linear} module, the \textbf{Non-Linearity} module, and the \textbf{Directed Interaction} module (\Figref{fig:model_detail}), enabling the network's structural richness and expressivity.

We will show that these modules properly tackled the defects in prior models and encourages efficient interactions within each network layer.

\cd{Given a scalar-vector tuple $(\vs,\mV)$, it is first passed into the Directed Linear module, the core part of a DW layer which synergistically lift the two input components $\vs$ and $\mV$ into latent features $\vt$ and $\mH$. The Non-Linear module is then applied, followed by the Directed Interaction module that integrates the two components in a biologically meaningful sense.}
\CD{Should we use $(\vt,\mH)$ for latent features and keep $\vh$ as $\mH$-entries?}

\cd{
\paragraph{Directed Linear module}
Key to the directed linear module is...
\begin{alignat}{3}
    \vt^{vs} &= \vecr{\mW}^{vs} \cdot \mV
    &&\quad\in \mathbb{R}^{C_h^s}
    \label{eqn:vs}
    \\
    \mH^{vv,c} &= \mW^{vv,cp}(\vecr{\mW}^{vv,cv}\times \mV) 
    &&\quad\in \R^{C_h^v \times 3}
    \label{eqn:vvc}
\end{alignat}
%
In addition, a directed weight can lift scalars to vectors by
\begin{alignat}{3}
    \mH^{sv} &= \vs\vecr{\mW}^{sv}
    &&\quad\in \mathbb{R}^{C_h^v\times 3}
    \label{eqn:sv}
\end{alignat}
%
Finally, we still allow taking linear combinations with standard weights for both scalar and vector components:
\begin{alignat}{3}
    \vt^{ss} &= \mW^{ss}\vs
    &&\quad\in \R^{C_h^s}
    \label{eqn:ss}
    \\
    \mH^{vv,p} &= \mW^{vv,p}\mV
    &&\quad\in \R^{C_h^v \times 3}
    \label{eqn:vvs}
\end{alignat}
}


Here $h^{ss}$ and $h^{vs}$ are scalars and $H^{sv}$, $H^{vv,p}$ and $H^{vv,c}$ are vectors for each sample. The operator $\times$ denotes the cross product of two 3-dimensional vectors. The scalar-to-scalar operation is the same as the standard neural network that applies a linear transformation on the input, with the weight matrix $\mW^{ss}$ of size $C_{h}^s\times C_\mathrm{in}^s$ (\Eqref{eqn:ss}). In \Eqref{eqn:vvs}, the superscript $p$, $c$ stands for projection and cross product, respectively. The weight matrices $\mW^{vv,p},\mW^{vv,cp}$ are of size $C_{h}^v\times C_\mathrm{in}^v$, and the directed weight matrix $\mW^{vv,cv}$ is of size $C_\mathrm{in}^s\times 3$. There are two different ways of transforming from vectors to vectors: 1) directly project a 3D vector to another hidden space by multiplying a tensor (\Eqref{eqn:vvs}); 2) a 3D vector cross-products a directed 3D weight matrix (\Eqref{eqn:vvc}). The key difference is that \Eqref{eqn:vvs} defines linear combinations of the input vectors. The output vector of two input vectors $v_1$ and $v_2$ can only lie in the plane $w_1v_1+w_2v_2$. In another hand, cross-product in \Eqref{eqn:vvc} creates a new direction outside the plane $w_1v_1+w_2v_2$, which is crucial in protein modelling. For instance, the side-chain angles of residue $i$ and $i+1$ are largely determined by the $c_\alpha-c_\beta$ vectors of residue $i$, which could lie outside the space containing these two vectors. In \Eqref{eqn:sv} and \Eqref{eqn:vs}, the directed weight matrices $\mW^{sv}_{x,y,z}\in\mathbb{R}^{3 \times C_{h}^s\times C_\mathrm{in}^v}$ and $\mW^{vs}_{x,y,z}\in\mathbb{R}^{3 \times C_{h}^v\times C_\mathrm{in}^s}$ represent their corresponding transformation on each coordinate component, and together forms the directed weights that facilitate information flow between scalars and vectors.

The output hidden representations from \Eqref{eqn:ss} to \Eqref{eqn:vvs} are concatenated and projected into one hidden space as the follows:

%\vspace{-1.5em}

\begin{alignat}{3}
    \vh^s&=\mW^{s}[\vh^{ss}\|\vh^{vs}] &&\quad\in \R^{C_h^s}\\
    \mH^v&=\mW^{v}[\mH^{sv}\|\mH^{vv,p}\|\mH^{vv,c}] &&\quad\in \R^{C_h^v\times 3}
\end{alignat}

\CD{I suggest comma instead $\|$ for concatenation. $\|$ looks like cross-entropy.}
Here $\|$ denotes the concatenation operation and the weight matrices $\mW^s,\mW^v$ have the dimensionality of $C_h^s\times 2C_h^s,C_h^v\times 3C_h^v$, respectively.

\cd{
\paragraph{Non-linearity module}
}
The scalar and vector representations are then fed into the \textbf{Non-linearity} module. For scalars, we use the ReLU function \cite{nair2010rectified} as the non-linear transformation. For vectors, we follow the previous work \cite{weiler20183d,jing2020learning,schutt2021equivariant} and multiply the hidden value by the sigmoid value of their feature-wise norms as follows.

%\vspace{-1.5em}

\begin{align}
\vh^s&\gets\mathrm{ReLU}(\vh^s)\\
h_{ij}^v&\gets h_{ij}^v\cdot\mathrm{sigmoid}(\|\vh_i^v\|)
\end{align}

\cd{
\paragraph{Directed Interaction module}
}

%\vspace{-0.5em}
Next we investigate how to efficiently integrate scalar and vector representations from previous layers to achieve more biological meaningful representations of the entire protein structure. We thus introduce the \textbf{Directed Interaction} layer as follows, 

%\vspace{-1.5em}

\begin{alignat}{3}
    \vb&=\mW^b_x\vh^v_x+\mW^b_y\vh^v_y+\mW^b_z\vh^v_z &&\quad\in \R^{C_h^s}\label{eqn:bias}\\
    \vs'&=\vh^s+\vb &&\quad\in \R^{C_h^s}\\
    \mC&=[\mW^c_x\vh^s,\mW^c_x\vh^s,\mW^c_x\vh^s]^\top &&\quad\in \R^{C_h^v\times 3}\label{eqn:coef}\\
    \mV'&=\mC \odot \mH^v &&\quad\in \R^{C_h^v\times 3}
\end{alignat}

Here $\mW^c_x,\mW^c_y,\mW^c_z$ have the size $C_h^v\times C_s^s$ and $\mW^b_x,\mW^b_y,\mW^b_z$ have the size $C_h^s\times C_h^v$. The operator $\odot$ denotes the elementwise product. In \Eqref{eqn:vvc} the new scalar representation $s'$ is a summation of the original scalar and a bias term which is a linear transformation of the vector representation. In this way, the output label could dynamically determine how much the prediction should rely on scalar and vector representations at this layer. However, this way cannot be adopted on the vector representation as it makes the model non-equivariant. Therefore, in \Eqref{eqn:coef}, we take the linear transformation of scalar features as the attention of the vector representation, which could be viewed as weighting multiple vectors using the scalar features. The entire Directed Interaction layer is another type of Nonlinearity layer.

\subsection{Equivariant Message Passing on Protein Graphs}
\label{emp}

\CD{We put our emphasis on the "versatility and compatibility" of DW on GNNs?}
\cd{
Classical GNNs don't allow scalar-vector communications and usually treat them as separate channels. TFN \cite{thomas2018tensor} propose a method to operate between $\mathrm{SO}(3)$-representations of different dimensions, but with learnable parameters only in a radial filter.
While providing a more flexible toolbox bridging scalar and vector channels, our DW network is also versatile enough to be plugged into any existing graph message passing paradigm, enriching them with geometrical or biological interpretations.
}

In this work, we represent a protein 3D structure as a proximity graph $\mathcal{G=(V,E)}$, where each node $u\in \mathcal{V}$ with edges connecting its k-nearest neighbors in 3D space. Here we use $h_u$ and $e_{uv}$ denote node and edge feature respectively, which can be either scalar or vector features.  The detailed scalar and vector features can be found in \Secref{pf}.


The Message Passing paradigm \cite{gilmer2017neural} is widely adopted in graph representation models to update node/edge representations by aggregating features from local neighbors, which has been demonstrated to be efficient in leveraging the graph structure information. Here, we find that the equivariant property could be easily achieved by transforming the coordinates of the atoms from the local frame of each residue to a global frame shared by the entire protein back and forth during the message passing process. In particular, we observe that the four backbone atoms of a residue in the protein structure form an intrinsic \textbf{rigid local frame}, which can be used to construct a local rotation matrix. We thus propose an Equivariant Message Passing algorithm to integrate the information on the protein graphs. We pre-compute the local rotation matrix $\mO_u \in \R^{3\times 3}$ for a residue $u$ using the four backbone atoms' coordinates $C_\beta^u,O^u,N^u,C_\alpha^u \in \R^3$, to perform the coordinate transformations on the hidden representations, $h=(\vs,\mV)$ between the global frame and the particular local frame of $u$ when updating its vector representation (\Eqref{frame}).

%\vspace{-2em}

\begin{align}
    \vx_u&=N^u-C_\alpha^u\\
    \vy_u&=C_\beta^u-C_\alpha^u \\
    \mO_u&=[\vx_u,\vy_u,\vx_u\times \vy_u]
    \label{frame}
\end{align}

%\vspace{-1em}

Then we can define $f_l$ and $f_g$ which transforms between the global frame to the local frame for residue $u$ back and forth as follows.

\vspace{-2em}

\begin{align}
    f_l(h,\mO_u) &:= (\vs,\mV \mO_u) \label{eqn:fl} \\
    f_g(h,\mO_u) &:= (\vs,\mV \mO_u^\top)
    \label{eqn:fg}
\end{align}

%\vspace{-0.5em}

Let $l$ be the index of the current layer of the integrated DW layer. The output of the DW layer is the concatenation of the resulted scalars and vectors along each channel dimension:

%\vspace{-1em}

\begin{equation}
    h_u\|h_v:=(\vs_u\|\vs_v,\mV_u\|\mV_v)
\end{equation}

%\vspace{-0.5em}

At the $l+1$th layer of the message passing, we first transform the vector representations of the each from the global frame to its local coordinate frame by using the pre-computed rotation matrix. Then we calculate the message for each edge $(u,v)\in\mathcal{E}$ by applying a sequential of Directed Weight perceptrons $\mathcal{F}$ on the concatenation of node features $h_u^l$, $h_v^l$ and edge feature $e_{uv}^l$. The messages are then aggregated over neighborhood $\mathcal{N}_u$ of node $u$(\Eqref{eqn:message}). Another Directed Weight perceptron $\mathcal{H}$ is applied to update the new node representation. In the end, we need to transform the representation defined in the local frame back to the global frame to preserve rotation equivariance (\Eqref{eqn:update}). The detailed proof of equivariance can be found in the appendix \Secref{pr}.

%\vspace{-1.0em}
\begin{align}
    m_{u}^{l+1}&=\sum_{v\in\mathcal{N}_u}\mathcal{F}(f_l(h_u^l\|h_v^l\|e_{uv}^l,\mO_u))\label{eqn:message}\\
    h_u^{l+1}&=f_g(\mathcal{H}(h_u^l\|m_u^{l+1}),\mO_u)
    \label{eqn:update}
\end{align}

\subsection{Variants of Directed Weight Graph Neural Networks}
\label{variants}

The Direct Weight layer is model-agnostic and can be integrated into multiple GNN frameworks. This is important because different variants of GNN models has been demonstrated to be helpful for different bioinformatics tasks involving protein 3D structures \cite{ingraham2019generative,strokach2020fast,baldassarre2021graphqa}. Therefore, we construct the DW layer into the following GNN variants to test their prediction performance.

\textbf{DW-GCN}. This is the one described and implemented in the previous subsection with \Eqref{eqn:message} and \Eqref{eqn:update}. 

\textbf{DW-GIN}. GIN is adopts the graph isomorphism operator \cite{xu2018powerful}. It is also straightforward to adopt both DW layer and Equivariant Message Passing framework on GIN as follows,

%\vspace{-2em}
\begin{align}
    m_u&=(1+\varepsilon)f_l(h_u,\mO_u)+\sum_{v\in\mathcal{N}_u}f_l(h_v,\mO_u) \\
    h'_u&=f_g\left(\mathcal{H}(m_u),\mO_u\right)
\end{align}

Here $\varepsilon$ is the learnable weighing parameter. $f_l$ and $f_g$ are the same transformation functions defined at \Eqref{eqn:fl} and \Eqref{eqn:fg}, and $\mathcal{H}$ is a multi-layer DW perceptron.

\textbf{DW-GAT}. In comparison to GCN and GIN, it is not trivial to incorporate DW layer to the Graph Attention Network (GAT)\cite{velivckovic2017graph}. In particular, the scalar and vector representations need to have their own attentions which are defined as follows,

\begin{align}
    (\vs_u,\mV_u)&= f_l(h_u,\mO_u)\\
    \vs'_u&=\sum_{v\in\mathcal{N}_u\cup\{u\}}\alpha^s_v \vs_v\\
    \mV'_u&=\sum_{v\in\mathcal{N}_u\cup\{u\}}\alpha^v_v \mV_v \\
    h'_u&=f_g((\vs',\mV'),\mO_u)
\end{align}

Here the attention scores $\alpha^s,\alpha^v$ are the softmax values over the inner products of all neighboring source-target pairs:
\begin{align}
    \alpha^s_v&=\frac{\exp{(\langle \vs_u,\vs_v\rangle)}}{\sum_{w\in\mathcal{N}_u\cup\{u\}}\exp{(\langle \vs_u,\vs_w\rangle)}}\\
    \alpha^v_v&=\frac{\exp{(\mathrm{tr}(\mV_u^\top \mV_v)}}{\sum_{w\in\mathcal{N}_u\cup\{u\}}\exp{(\mathrm{tr}(\mV_u^\top \mV_v))}}
\end{align}

For scalar representations, the standard inner product is used. For vector representations, the Frobenius inner product $\langle \mV_u,\mV_v\rangle=\mathrm{tr}(\mV_u^\top \mV_v)$ is used because they are tensors.



==> tables/results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\begin{tabular}{|l|l|}
\hline
\multicolumn{1}{|c|}{Method} & Recovery\%                  \\ \hline
DenseCPD                     & 50.7                        \\ \hline
ProDCoNN                     & {\color[HTML]{000000} 40.7} \\ \hline
SBROF                        & 39.2                        \\ \hline
SPIN2                        & 33.6                        \\ \hline
Wang's model                 & 33.0                        \\ \hline
ProteinSolver                & 30.8                        \\ \hline
SPIN                         & 30.3                        \\ \hline
Rosetta                      & 30.3                        \\ \hline
GVP-GNN                      & 44.9                        \\ \hline
DWNN                         & \textbf{51.5}               \\ \hline
\end{tabular}
\caption{We test some variants of attack location search methods on AG-news dataset.POS means only using pos\_tags to find the locations to be attacked and PR is the search method we use.Result shows that PR is more efficient than others.}
\label{tab:ex2}
\end{table}








